A Rapidly-Exploring Random Trees Motion Planning Algorithm for Hybrid Dynamical Systems

This paper proposes a rapidly-exploring random trees (RRT) algorithm to solve the motion planning problem for hybrid systems. At each iteration, the proposed algorithm, called HyRRT, randomly picks a state sample and extends the search tree by flow or jump, which is also chosen randomly when both regimes are possible. Through a definition of concatenation of functions defined on hybrid time domains, we show that HyRRT is probabilistically complete, namely, the probability of failing to find a motion plan approaches zero as the number of iterations of the algorithm increases. This property is guaranteed under mild conditions on the data defining the motion plan, which include a relaxation of the usual positive clearance assumption imposed in the literature of classical systems. The motion plan is computed through the solution of two optimization problems, one associated with the flow and the other with the jumps of the system. The proposed algorithm is applied to a walking robot so as to highlight its generality and computational features.

==> analysis_on_newstate.tex <==
\section{Analysis on the Different Implementation of $new\_state$ Function }
\label{section:caseanalysisontwomethods}
In Section \ref{section:newstate}, two different methods of implementing $new\_state$ function are stated.  This section analyzes the differences between two different implementation. The sample motion planning problems for bouncing ball system and actuated point mass system are used as test problems for both implementation, denoted $\mathcal{P}_{bb}$ and $\mathcal{P}_{apm}$. Two RRT-based planner, Planner A and Planner B, are given. Planner A implements the $new\_state$ function by randomly picking an input value/input signal from input library. Planner B implements the $new\_state$ function by solving the optimization problems. The rest of the setting of Planner A and B are same. 
\subsection{Success rate}
The two test problems are solved for $100$ times, by both Planner A and Planner B.  Planner A succeeds in finding a motion plan to $\mathcal{P}_{bb}$ for $87$ times. Planner B succeeds in finding a motion plan to $\mathcal{P}_{bb}$ for all $100$ times. Planner A succeeds in finding a motion plan to $\mathcal{P}_{apm}$ for $26$ times. Planner B succeeds in finding a motion plan to $\mathcal{P}_{apm}$ for $21$ times. The table of success rate for each planner solving each test problem is given in Table \ref{table:successrate}. The different implementation of $new\_state$ function does not affect if the planner finds a motion plan within a fixed iteration 
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{ ccc } 
			Success rate & $\mathcal{P}_{bb}$ & $\mathcal{P}_{apm}$ \\ 
			\hline
			Planner A & $87\%$ &  $26\%$\\ 
			Planner B & $100\%$ & $21\%$ \\ 
			\hline
		\end{tabular}
	\end{center}
	\label{table:successrate}
	\caption{Success rate}
\end{table}
\subsection{Average number of iteration and number of generated vertices}
In the instances when Planner A succeeds in finding a motion plan to $\mathcal{P}_{bb}$, Planner A iterates for $251$ times and generates $47$  vertices during the search. In the instances when Planner B succeeds in finding a motion plan to $\mathcal{P}_{bb}$, Planner B iterates for $188$ times and generates $33$  vertices during the search. In the instances when Planner A succeeds in finding a motion plan to $\mathcal{P}_{apm}$, Planner A iterates for $558$ times and generates $155$  vertices during the search. In the instances when Planner B succeeds in finding a motion plan to $\mathcal{P}_{apm}$, Planner B iterates for $488$ times and generates $41$  vertices during the search. The statistics results are shown in Table \ref{table:iterationnumber} and \ref{table:generatedvertices}.
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{ ccc } 
			Iteration number & $\mathcal{P}_{bb}$ & $\mathcal{P}_{apm}$ \\ 
			\hline
			Planner A & $251$ &  $558$\\ 
			Planner B & $188$ & $488$ \\ 
			\hline
		\end{tabular}
	\end{center}
	\label{table:iterationnumber}
	\caption{Iteration number}
\end{table}

\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{ ccc } 
			Generated vertices number & $\mathcal{P}_{bb}$ & $\mathcal{P}_{apm}$ \\ 
			\hline
			Planner A & $47$ &  $155$\\ 
			Planner B & $33$ & $41$ \\ 
			\hline
		\end{tabular}
	\end{center}
	\label{table:generatedvertices}
	\caption{Generated vertices number}
\end{table}

This statistics result shows that the RRT-based planner that implements $new\_state$ function using optimization-based method iterates for fewer times and generates fewer vertices when a motion plan is obtained, compared with the RRT-based planner that implements $new\_state$ function by randomly pick. The fewer number of vertices are generated, the less memory are used to store the intermediate results. However, the smaller number of iteration does not necessarily mean the less time consumption, since Planner B takes more time at each iteration to solve the optimization problems.

\subsection{Time consumption}
The time consumption for each test is shown in Table \ref{table:timeconsumption}. The statistics shows that although Planner A and B spend almost the same time on average to solve $\mathcal{P}_{bb}$, Planner A spends significantly less time in solving $\mathcal{P}_{apm}$ than Planner B. This indicates that the RRT-based planner that implements $new\_state$ function using random pick can eventually be more efficient in solving some motion planning problem, compared with the planner that implements $new\_state$ function by solving optimization problems.
\begin{table}[htbp]
	\begin{center}
		\begin{tabular}{ ccc } 
			Time consumption & $\mathcal{P}_{bb}$ & $\mathcal{P}_{apm}$ \\ 
			\hline
			Planner A & $1.11$  seconds&  $4.29$ seconds\\ 
			Planner B & $1.01 $ seconds& $8.63$ seconds \\ 
			\hline
		\end{tabular}
	\end{center}
	\label{table:timeconsumption}
	\caption{Time consumption}
\end{table}





%%% BIBLIOGRAPHY


%




==> continuoussimulator.tex <==
\section{Simulator of continuous dynamics}
\label{section:flowsystemsimulator}
The proposed algorithm requires a simulator to simulate a solution pair starting from a given initial state $x_{0}\in C'$ with a given input signal $\tilde{u}\in \mathcal{U}_{C}$ applied, following continuous dynamics. Since the simulator follows the continuous dynamics of the hybrid system, the initial state $x_{0}$, flow set $C$ and flow map $f$ are fed into the system simulator. 

Note that when the simulated solution enters the intersection between flow set $C$ and jump set $D$, it can either keep flowing or stop to jump. In \cite{sanfelice2013toolbox}, the hybrid system simulator HyEQ uses a scalar parameter $rule$ to define whether the simulator gives priority to jumps ($rule= 1$), priority to flows ($rule= 2$), or no priority ($rule= 3$) when both $x\in C$ and $x\in D$ hold. When no priority is selected, then the simulator selects flowing or jumping randomly.
	
	Therefore, the jump set $D$ and a priority option $rule$  should be fed to the system simulator. If $rule = flow$,  the simulated solution will keep flowing. If $rule = jump$, the simulated solution will stop. In this paper, the option of random selection is not considered.  Therefore, the proposed simulator should be able to solve the following problem.
\begin{problem}
	\label{problem:flowsimulator}
	Given the flow set $C$, flow map $f$ and jump set $D$ of a hybrid system $\mathcal{H}$ with input $u\in \mathbb{R}^{m}$, state $x\in \mathbb{R}^{n}$, a priority option flag $rule\in \{flow, jump\}$, an initial state $x_{0}\in \mathbb{R}^{n}$ and an input signal $\tilde{u}\in \mathcal{U}_{C}$ such that $(x_{0}, \tilde{u}(0))\in C$, find a pair $(\phi, u):  [0, t^{*}]\times \{0\} \to \mathbb{R}^{n} \times \mathbb{R}^{m}$, where $t^{*}\in [0, \overline{t}(\tilde{u})]$, such that the following hold:
	\begin{enumerate}
		\item $\phi(0, 0) = x_{0}$;
		\item For all $t\in [0, t^{*}]$, $u(t, 0) = \tilde{u}(t)$;
		\item If $[0, t^{*}]$ has nonempty interior,
		\begin{enumerate}
			\item the function $t\mapsto \phi(t, 0)$ is locally absolutely continuous,
			\item for all $t\in (0, t^{*})$,
				\begin{equation}
					\begin{aligned}
					(\phi(t, 0),u(t, 0))&\in C & \text{ if }rule = flow\\
					(\phi(t, 0),u(t, 0))&\in C\backslash D &\text{ if }rule = jump,\\
					\end{aligned}
				\end{equation}
			\item for almost all $t\in [0, t^{*}]$,
			\begin{equation}
			\label{equation:differentialequation}
			\dot{\phi}(t,0) = f(\phi(t,0), u(t,0)).
			\end{equation}
		\end{enumerate}
	\end{enumerate}
\end{problem}
\begin{remark}
	The solution to Problem \ref{problem:flowsimulator} is not unique. If there exists a solution $(\phi, u)$ to Problem \ref{problem:flowsimulator}, then for any hybrid time $(t_{1}, j_{1})\in \dom (\phi, u)$, the truncation of $(\phi, u)$ between $(0, 0)$ and  $(t_{1}, j_{1})$ is also a solution to Problem \ref{problem:flowsimulator}. The definition of truncation operation is provided in Definition \ref{definition: truncation}.
\end{remark}
In this paper, the simulator is designed to simulate the maximal solution to Problem \ref{problem:flowsimulator}. The definition of maximal solution is given as follows. 
\begin{definition}
	(Maximal solution) A solution $\psi$ to Problem \ref{problem:flowsimulator} is said to be maximal if there does not exist another solution $\psi'$ to Problem \ref{problem:flowsimulator} such that $\dom \psi$ is a proper subset of $\dom \psi'$ and $\psi(t, 0) = \psi'(t, 0)$ for all $t\in \dom_{t} \psi$.
\end{definition}

The module to simulate the maximal solution to Problem \ref{problem:flowsimulator} is called simulator of continuous dynamics. As is shown in Figure \ref{fig:flowsimulator}, the input of this module is flow set $C$, flow map $f$, jump set $D$, priority option flag $rule$, initial state $x_{0}$ and input signal $\tilde{u}$. The output of this module is the maximal solution $(\phi, u)$ to Problem \ref{problem:flowsimulator} given the data above. Therefore, this module can be denoted as
\begin{equation}
\label{model:flowsystemsimulator}
(\phi, u) = continuous\_simulator(C, f, D, rule,  x_{0}, \tilde{u}).
\end{equation}

\begin{figure}[htbp] 
	\centering
	\incfig[1.1]{flowsimulator} 
	\caption{A simulator of continuous dynamics }\label{fig:flowsimulator} 
\end{figure} 

The maximal solution to Problem \ref{problem:flowsimulator} can be simulated in the following steps. 
\begin{steps}
	\item Construct a helper function $\hat{\phi}: [0, \overline{t}(\tilde{u})]\to \mathbb{R}^{n}$ by
	\begin{equation}
	\label{equation:flowequationintegration}
			\hat{\phi}(t) = x_{0} + \int_{0}^{t}f(\hat{\phi}(\tau),\tilde{u}(\tau))d\tau \quad t\in [0, \overline{t}(\tilde{u})].
	\end{equation} 
	\item Determine the time $\hat{t}\in [0, \overline{t}(\tilde{u})]$ by
	\begin{equation}
	\label{equation:integrationduration}
		\hat{t} = \left\{\begin{aligned}
			\begin{aligned}
			\max \{t&\in [0, \overline{t}(\tilde{u})]: \forall t'\in (0, t), (\hat{\phi}(t'), \tilde{u}(t'))\\ &\in C\}  \qquad \text{ if } rule = flow\\
			\max \{t&\in [0, \overline{t}(\tilde{u})]: \forall t'\in (0, t), (\hat{\phi}(t'), \tilde{u}(t'))\\ &\in C\backslash D\}  \qquad\text{ if } rule = jump.\\
			\end{aligned}
		\end{aligned}
		\right.
	\end{equation}
	\item Construct the solution function pair $(\phi, u): [0, \hat{t}]\times \{0\}\to \mathbb{R}^{n}\times \mathbb{R}^{m}$ by 
	\begin{equation}
	\label{equation:flowsegment}
		\begin{aligned}
			\phi(t, 0) &= \hat{\phi}(t)\quad t\in [0, \hat{t}]\\
			u(t, 0) &= \tilde{u}(t)\quad t\in [0, \hat{t}].\\
		\end{aligned}
	\end{equation}
\end{steps}
The solution function pair $(\phi, u)$ is the maximal solution to Problem \ref{problem:flowsimulator} and hence the output of module $continuous\_simulator$. Note that the challenge in implementing Step 1 is the integration in (\ref{equation:flowequationintegration}). It can be approximated by employing numerical integration methods. The challenge in implementing Step 2 is determining $\hat{t}$ in (\ref{equation:integrationduration}) during the integration. It can be approximated by employing zero-crossing detection algorithms. \textcolor{red}{Next, we discuss} how numerical integration scheme and zero-crossing detection algorithm are modeled, following a computational approach to implement the simulator of continuous dynamics.

\input{section_numerical_integration}
\input{section_zero_crossing_detection}
\input{section_computation_framework}

==> discretesimulator.tex <==
\subsection{Simulator of discrete dynamics}
　\label{section:jumpsystemsimulator}
　The proposed algorithm requires a system simulator to simulate a purely discrete solution pair with a single jump, starting from an initial state $x_{0}\in D'$ with an input $u_{D}\in \mathcal{U}_{D}$ applied. Namely, the system simulator should be able to solve the following problem:
　\begin{problem}
	\label{problem:jumpsimulator}
	Given the jump set $D$ and jump map $g$ of hybrid system $\mathcal{H}$ with input $u\in \mathbb{R}^{m}$, state $x\in \mathbb{R}^{n}$, an initial state $x_{0}\in \mathbb{R}^{n}$ and an input value $u_{D}\in \mathcal{U}_{D}$ such that $(x_{0}, u_{D})\in D$, find a pair $(\phi, u):  \{0\}\times \{0, 1\} \to \mathbb{R}^{n} \times \mathbb{R}^{m}$ such that the following hold:
　	\begin{enumerate}
		\item $\phi(0, 0) = x_{0}$;
　		\item $u(0, 0) = u_{D}$;
　		\item $\phi(0, 1) = g(\phi(0, 0), u(0, 0))$.
	\end{enumerate}
\end{problem}
Problem \ref{problem:jumpsimulator} can be solved by constructing a function pair $(\phi, u):  \{0\}\times \{0, 1\} \to \mathbb{R}^{n} \times \mathbb{R}^{m}$ such that
\begin{equation}
\label{equation:jumpsegment}
\begin{aligned}
\phi(0, 0) &= x_{0}\\
\phi(0, 1) &= g( x_{0}, u_{D})\\
u(0, 0) & = u_{D}\\
u(0, 1)  & \in \mathbb{R}^{m}.
\end{aligned}
\end{equation}
In (\ref{equation:jumpsegment}), $u(0, 1)  \in  \mathbb{R}^{m}$ can be implemented by selecting an element in $ \mathbb{R}^{m}$ and assigning the element to $u(0, 1)$. The selection can be made by choosing a fixed value or simple random sampling in $\mathbb{R}^{m}$. The selection should avoid the input values such that $(\phi(0, 1), u(0, 1))$ falls into unsafe set. 

The construction in (\ref{equation:jumpsegment}) can be seen as a module called simulator of discrete dynamics. As is shown in Figure \ref{fig:jumpsimulator}, the inputs of this module are jump set $D$, jump map $g$, initial state $x_{0}\in D'$ and input $u_{D}\in \mathcal{U}_{D}$ such that $(x_{0}, u_{D})\in D$. The output of this module is the solution pair $(\phi, u)$ constructed in (\ref{equation:jumpsegment}). Therefore, the module can be denoted as
\begin{equation}
\label{model:jumpsystemsimulator}
(\phi, u) = discrete\_simulator(D, g, x_{0}, u_{D}).
\end{equation}

\begin{figure}[htbp] 
	\centering
	\incfig[1.2]{jumpsimulator} 
	\caption{Simulator of discrete dynamics }\label{fig:jumpsimulator} 
\end{figure} 

==> inputsignals.tex <==
\section{Input library}
\label{section:inputlibrary}
The proposed algorithm requires a library of inputs such that the algorithm can apply the inputs therein to simulate solution pairs. Note that inputs are constrained by the flow set $C$ and jump set $D$, respectively. Given flow set $C$ and jump set $D$ of the hybrid system $\mathcal{H}$, the input signal set during flows, denoted  $\mathcal{U}_{C}$, and input set at jumps, denoted $\mathcal{U}_{D}$, are described as follows. 
\begin{enumerate}
	\item The input signal applied during the flows is a continuous-time signal. Therefore, the input signal during flows, denoted $\tilde{u}$, is specified by a function from an interval of time of the form $[0, t^{*}]$ to $U_{C}$ for some $t^{*}\in \mathbb{R}_{\geq 0}$, namely,
	$$
	\tilde{u}: [0, t^{*}]\to U_{C}.
	$$
	Definition \ref{definition:solution} also requires that $\tilde{u}$ is Lebesgue measurable and locally bounded.
	Then, input signal set during flows, denoted $\mathcal{U}_{C}$, is a pre-determined set that collects possible $\tilde{u}$ that can be applied during flows. 
	
	Given $\tilde{u}\in\mathcal{U}_{C}$, the functional $\overline{t}: \mathcal{U}_{C} \to [0, \infty)$ returns the time duration of $\tilde{u}$. Namely, given any $\tilde{u}: [0, t^{*}]\to U_{C}$, $\overline{t}(\tilde{u}) = t^{*}$.
	\item The input applied at a single jump can be specified by an input value in $U_{D}$. Input set at jumps, denoted $\mathcal{U}_{D}$, is a pre-determined set that collects possible values of input that can be applied at jumps, namely, 
	$$
		\mathcal{U}_{D}\subset U_{D}.
	$$
\end{enumerate}
The pair of sets $(\mathcal{U}_{C}, \mathcal{U}_{D})$ defines the input library, denoted $\mathcal{U}$, namely,
$$
	\mathcal{U} := (\mathcal{U}_{C}, \mathcal{U}_{D}).
$$

\label{section:samplingmotionprimitives}
The following introduces a method to construct $\mathcal{U}_{C}$ and $\mathcal{U}_{D}$, given sets $C$ and $D$ respectively. The  procedure to construct $\mathcal{U}_{C}$ is given as follows.
\begin{steps}
	\item Set $t^{*}$ to a positive constant. Choose a finite number of elements from $U_C$ and denote it $U^s_C$.
	\item For each $u^{s}\in U_{C}^{s}$, construct an input signal $[0, t^{*}]\to \{u^{s}\}$ and add it to $\mathcal{U}_{C}$. 
\end{steps}
The construction of $\mathcal{U}_{D}$ can be implemented by choosing a finite number of elements from $U_{D}$. 

The method of choosing elements from $U_{C}$ and $U_{D}$ varies when solving different motion planning problems. An example of constructing $\mathcal{U}_{C}$ and $\mathcal{U}_{D}$ to solve the sample motion planning problem for bouncing ball system is given as follows.
\begin{example}
	 (Bouncing ball system in Example \ref{example:bouncingball}, revisited) In the sample problem in Example \ref{example:bouncingball}, since $X_{u} =\{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: u\in[5, \infty)\}$, the input values in $[5, \infty)$ are unsafe.  Because $C = \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1}\geq 0\}$, then $U_{C} = \mathbb{R}$.  Note that the input does not affect flow map. Hence,  any input values in the interval $(-\infty, 5)$ can be chosen as the elements of $U_{C}^{s}$. For example, $U_{C}^{s}$ is constructed as $\{0\}$ in the forthcoming illustration in Section \ref{section:illustrationbb}. When $t^{*} = 0.1$, an input signal $[0, 0.1]\to \{0\}$ is constructed and added to $\mathcal{U}_{C}$.
	 
	 The jump set of the bouncing ball system is $D= \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1} = 0, x_{2} \leq 0, u\geq 0\}$. Therefore,  $U_{D} = [0, \infty)$. Considering the inputs in $[5, \infty)$ are unsafe, the elements in $\mathcal{U}_{D}$ can be chosen from the interval $[0, 5)$. For example, $\mathcal{U}_{D}$ is constructed as $\{0, 1, 2, 3, 4\}$ in the forthcoming illustration in Section \ref{section:illustrationbb}.
\end{example}

==> lemma_flow.tex <==




==> probablistic_completeness.tex <==
\subsection{Probabilistic completeness}
Probabilistic completeness is an important property for the randomized planning algorithm like RRT algorithm. It indicates that when the number of iteration goes to infinite, the probability of finding a solution is approaching to $1$. 

Whether a RRT-based planner is able to find a motion plan depends on if a state $x_{0}^{s}$ is sampled when initializing the search graph such that there exists a motion plan that starts from $x_{0}^{s}$. It also depends on if the input signals in the input signal libraries are sufficient to describe the input trajectory during the flows and at jumps. Therefore, Assumption \ref{assumption:inputsignallibrary} is imposed on the sampling in the initial state set and the constructed input signal library.
\begin{assumption}
	\label{assumption:inputsignallibrary}
	When a RRT-based planner is used to solve a motion planning problem $\mathcal{P}$ with input signal libraries denoted as $\mathcal{U} = (\mathcal{U}_{C}, \mathcal{U}_{D})$, there exists a motion plan $\psi = (\phi, u)$ to $\mathcal{P}$ such that the following are satisfied:
	\begin{enumerate}
		\item  when initializing the search graph, there exists a sample $x_{0}^{s}\in X_{0}^{s}$ such that $\phi(0, 0) = x_{0}^{s}$.
		\item for all $j\in \mathbb{N}$ such that $I^{j}$ has nonempty interior, there exists a sequence $(\tilde{u}^{C}_{i})_{i = 0}^{m}$, where $m$ is a positive integer or infinite, such that
		\begin{enumerate}
			\item $\tilde{u}^{C}_{i}\in \mathcal{U}_{C}$ for $i = 0, 1,..., m$;
			\item for all $t\in \interior I^{j}$, 
			\begin{equation}
			u(t, j) = \tilde{u}^{C}(t - T)
			\end{equation} where $\tilde{u}^{C} = \tilde{u}^{C}_{0}\circ\tilde{u}^{C}_{1}\circ... \circ \tilde{u}^{C}_{m}$ and $T = \min  I^{j} $.
			%			\begin{equation}
			%				T = \left\{\begin{aligned}
			%				&0 & j = 0\\
			%			    &\max I^{j - 1} & j \geq 1.\\
			%				\end{aligned}\right.
			%			\end{equation}
		\end{enumerate}
		\item for all $(t, j)\in \dom \psi$ such that $(t, j + 1)\in \dom \psi$, there exists a $\tilde{u}^{D}\in \mathcal{U}_{D}$ such that
		\begin{equation}
		u(t, j) = \tilde{u}^{D}(0).
		\end{equation}
	\end{enumerate}
\end{assumption}
\begin{remark}
	This assumption firstly guarantees that when sampling in the initial state set $X_{0}$ at the initialization step, one of the samples equals the initial state of the existing motion plan. This assumption also guarantees that the input signals in $\mathcal{U}_{C}$ and $\mathcal{U}_{D}$ are sufficient to solve the problem $\mathcal{P}$. More precisely, this assumption guarantees that the input trajectory of the motion plan during flows can be provided by the concatenation of input signals in  $\mathcal{U}_{C}$. It also guarantees that the input at jumps can also be provided by the input signals in $\mathcal{U}_{D}$. Therefore, there exists a sequence of input signals $\tilde{u}_{1}$, $\tilde{u}_{2}$, ..., $\tilde{u}_{k}$ that when applied to a sample $x_{0}^{s} = \phi(0, 0)$ in the initial state set $X_{0}$ yield a sequence of states $x_{0}$, $x_{1}$, ..., $x_{k + 1}\in X_{f}$. In other words, if $\tilde{u}_{1}$, $\tilde{u}_{2}$, ..., $\tilde{u}_{k}$ are applied sequentially to the hybrid system, starting from the sample $x_{0}^{s}$, the resulting solution pair is a motion plan to the given motion planning problem.
\end{remark}
Then the following establishes the probabilistic completeness of the RRT-based planner for hybrid system.
\begin{theorem}
	If the initialization of the search graph and the construction of input signal libraries for the RRT-based planner satisfy Assumption \ref{assumption:inputsignallibrary}, then the probability that the RRT will contain a state in $X_{f}$ as a vertex approaches $1$ as the number of vertices approaches infinity.
\end{theorem}
\begin{proof}
	Since Assumption \ref{assumption:inputsignallibrary} is satisfied, then there exists a sequence of input signals $\tilde{u}_{1}$, $\tilde{u}_{2}$, ..., $\tilde{u}_{k}$ that when applied to a state $x_{0}\in X_{0}$ yield a sequence of states $x_{0}$, $x_{1}$, ..., $x_{k + 1}\in X_{f}$. 
	
	This theorem is proved by induction. Assume that the existing search graph contains $x_{i}$ as a vertex after some finite number of iterations. Consider the Voronoi diagram associate with the states of the RRT vertices.  There exists a positive real number $c_{1}$ such that $\mu(Vor(x_{i}))> c_{1}$ where $\mu(S)$ denotes the probability of the event that sample lies in the region $S$. If a sample falls within the Voronoi region associated with $x_{i}$, then the vertex that represents $x_{i}$ will be selected. There exists a second positive number $c_{2}$ related to $c_{1}$ such that the probability that the correct input $u_{i}$ is selected is at least $c_{2}$. If both $x_{i}$ and $u_{i}$ have a probability of at least $c_{2}$ of being selected, the probability of event $E_{n}$ that both $x_{i}$ and $u_{i}$ are selected in one of the $n$ number of iterations is
	\begin{equation}
	\mu(E_{n}) = 1 - (1 - c_{2})^{n}.
	\end{equation} 
	Therefore,
	\begin{equation}
	\lim_{n\to \infty} \mu(E_{n}) = 1.
	\end{equation}
	In other words, when the number of iteration $n$ is approaching to infinity, the probability that both $x_{i}$ and $u_{i}$ are selected in one of these iterations is approaching to $1$.
	This argument can be applied inductively from $x_{i}$ to $x_{k}$ until the final state $x_{k + 1}\in X_{f}$ is reached.
\end{proof}

==> searchtree.tex <==
%\section{Search tree}
%\label{section:searchgraph}
%\label{section:graphrelated}
%A search tree of hybrid system $\mathcal{H}$ is directed acyclic graph from graph theory. A tree $\mathcal{T}$ is a pair $\mathcal{T} = (V, E)$, where $V$ is a set whose elements are called vertices and $E$ is a set of paired vertices whose elements are called edges. The edges in the directed tree are directed, which means the pairs of vertices that represent edges are ordered. Hence, the set of edges $E$ is defined as
%$$
%E \subseteq \{(v_{1}, v_{2}): v_{1}\in V, v_{2}\in V, v_{1}\neq v_{2}\}.
%$$
%The edge $e = (v_{1}, v_{2})\in E$ represents an edge from $v_{1}$ to $v_{2}$. 
%
%A path in $\mathcal{T} = (V, E)$ is a sequence of vertices
%\begin{equation}
%p = (v_{1}, v_{2}, ..., v_{k})
%\end{equation} such that $(v_{i}, v_{i + 1})\in E$ for all $i= 1, 2,..., k - 1$.
%
%%A vertex $v_{l}$ is said to be a leaf vertex in the graph $\mathcal{G} = (V, E)$ if there is no $v^*\in V$ such that $(v_{l}, v^*)\in E$.
%
%Each vertex $v\in V$ in the search tree of $\mathcal{H}$ represents a state $x\in \mathbb{R}^{n}$. Each edge $e = (v_{1}, v_{2})\in E$ represents a solution pair of $\mathcal{H}$  that starts from the state represented by $v_{1}$ and ends at the state represented by $v_{2}$. 
%
%In order to access the states and solution pairs that vertices and edges represent, functions $\overline{x}$ and $\overline{\psi}$ are defined. Given a vertex $v$, the function $\overline{x}$ returns the state that $v$ represents. Given an edge $e$, the function $\overline{\psi}$ returns the solution pair that $e$ represents.
%%Therefore, edge $(v_{1}, v_{2})$ represents a 
%%
%%Let $\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2})$ denote the set of solution pairs that starts from $x_{1}$ and ends with $x_{2}$. In other words, 
%%$$
%%\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2}): = \{\psi = (\phi, u): \psi \in \mathcal{S}_{\mathcal{H}}(x_{1}), \phi(T, J) = x_{2}, \text{where } (T, J) = \max \dom \psi\}
%%$$ 
%%where $\mathcal{S}_{\mathcal{H}}(x_{0})$ is the set of solution pairs $\psi = (\phi, u)$ of $\mathcal{H}$ such that $\phi(0, 0) = x_{0}$. Then 
%%$$
%%\overline{\mathcal{S}}_{\mathcal{H}}(X_{0}) := \bigcup_{x_{1}\in \mathcal{R}(X_{0}), x_{2}\in \mathcal{R}(X_{0}), x_{1}\neq x_{2}}\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2}).
%%$$
%%% where $\mathcal{R}_{\mathcal{H}}(X_{0})$ is the reachable set from $X_{0}$, as is defined in Definition \ref{definition:reachability}.
%
%%A search graph $\mathcal{G} = (V, E)$ is equipped with two maps:
%%\begin{itemize}
%%	\item $\overline{x}: V\to \mathcal{R}(X_{0})$, where $\overline{x}(v)$ returns the state represented by vertex $v$;
%%	\item $\overline{\psi}: E\to\overline{\mathcal{S}}_{\mathcal{H}}(X_{0}) $, where $\overline{\psi}(e)$ returns the solution pairs represented by edge $e$. 
%%\end{itemize} 
%
%Given a path 
%$$
%p = (v_{1}, v_{2}, ..., v_{k})
%$$ in the search tree $\mathcal{T} = (V, E)$, the function pair $\psi = (\phi, u)$ that $p$ represents is
%$$
%\psi = (\phi, u) = \overline{\psi}(e_{1})| \overline{\psi}(e_{2}) |...| \overline{\psi}(e_{k-1})
%$$
%where $e_{i} := (v_{i}, v_{i + 1})$ for all $i = 1, 2, ..., k - 1$ and the operator $|$ denotes the concatenation operation as is defined in Definition \ref{definition:concatenation}.
%In order to access the function pair that a path represents,  given a path 
%$$
%p = (v_{1}, v_{2}, ..., v_{k}),
%$$ a function $\tilde{\psi}$ is defined such that 
%\begin{equation}
%\tilde{\psi}(p) := \overline{\psi}((v_{1}, v_{2}))| \overline{\psi}((v_{2}, v_{3})) |...| \overline{\psi}((v_{k-1}, v_{k})).
%\end{equation}
%
%The reached set of a search tree $\mathcal{T} = (V, E)$, denoted $X_{\mathcal{T}}$, is defined as
%\begin{equation}
%\label{equation:reachedset}
%X_{\mathcal{T}} := \bigcup_{v\in V} \{\overline{x}(v)\}
%\end{equation}
%which includes all states represented by the vertices in search tree $\mathcal{T}$.


\subsection{Search tree}
\label{section:searchgraph}
%A search tree of hybrid system $\mathcal{H}$ is directed graph from graph theory. Each vertex $v\in V$ in the search graph of $\mathcal{H}$ represents a state $x\in \mathbb{R}^{n}$. Each edge $e = (v_{1}, v_{2})\in E$ represents a solution pair of $\mathcal{H}$  that starts from the state represented by $v_{1}$ and ends at the state represented by $v_{2}$. 
%A graph $\mathcal{G}$ is a pair $\mathcal{G} = (V, E)$, where $V$ is a set whose elements are called vertices and $E$ is a set of paired vertices whose elements are called edges. The edges in the directed graph are directed, which means the pairs of vertices that represent edges are ordered. Hence, the set of edges $E$ is defined as
%$$
%E \subseteq \{(v_{1}, v_{2}): v_{1}\in V, v_{2}\in V, v_{1}\neq v_{2}\}.
%$$
%The edge $e = (v_{1}, v_{2})\in E$ represents an edge from $v_{1}$ to $v_{2}$. 

%A vertex $v_{l}$ is said to be a leaf vertex in the graph $\mathcal{G} = (V, E)$ if there is no $v^*\in V$ such that $(v_{l}, v^*)\in E$.

Note that in the search tree $\mathcal{T} = (V, E)$, each vertex is associated with a state and each edge is associated with a solution pair.
Given a vertex $v\in V$, $\overline{x}(v)$ denotes the state associated with $v$. Given an edge $e\in E$, $\overline{\psi}(e)$ denotes the solution pair associated with $e$.
%Therefore, edge $(v_{1}, v_{2})$ represents a 
%
%Let $\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2})$ denote the set of solution pairs that starts from $x_{1}$ and ends with $x_{2}$. In other words, 
%$$
%\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2}): = \{\psi = (\phi, u): \psi \in \mathcal{S}_{\mathcal{H}}(x_{1}), \phi(T, J) = x_{2}, \text{where } (T, J) = \max \dom \psi\}
%$$ 
%where $\mathcal{S}_{\mathcal{H}}(x_{0})$ is the set of solution pairs $\psi = (\phi, u)$ of $\mathcal{H}$ such that $\phi(0, 0) = x_{0}$. Then 
%$$
%\overline{\mathcal{S}}_{\mathcal{H}}(X_{0}) := \bigcup_{x_{1}\in \mathcal{R}(X_{0}), x_{2}\in \mathcal{R}(X_{0}), x_{1}\neq x_{2}}\mathcal{s}_{\mathcal{H}}(x_{1}, x_{2}).
%$$
%% where $\mathcal{R}_{\mathcal{H}}(X_{0})$ is the reachable set from $X_{0}$, as is defined in Definition \ref{definition:reachability}.

%A search graph $\mathcal{G} = (V, E)$ is equipped with two maps:
%\begin{itemize}
%	\item $\overline{x}: V\to \mathcal{R}(X_{0})$, where $\overline{x}(v)$ returns the state represented by vertex $v$;
%	\item $\overline{\psi}: E\to\overline{\mathcal{S}}_{\mathcal{H}}(X_{0}) $, where $\overline{\psi}(e)$ returns the solution pairs represented by edge $e$. 
%\end{itemize} 
%Given a path 
%$
%p = (v_{1}, v_{2}, ..., v_{k})
%$ in the search tree $\mathcal{T} = (V, E)$, the function pair that $p$ represents is
%$$
%\overline{\psi}(e_{1})| \overline{\psi}(e_{2}) |...| \overline{\psi}(e_{k-1})
%$$
%where $e_{i} := (v_{i}, v_{i + 1})$ for all $i = 1, 2, ..., k - 1$ and the operator $|$ denotes the concatenation operation, as is defined in Definition \ref{definition:concatenation}.
%Given a path 
%$$
%p = (v_{1}, v_{2}, ..., v_{k}),
%$$ $\tilde{\psi}(p)$ denotes the function pair that $p$ represents, i.e., 
%$$
%\tilde{\psi}(p)  := \overline{\psi}((v_{1}, v_{2}))| \overline{\psi}((v_{2}, v_{3})) |...| \overline{\psi}((v_{k-1}, v_{k})).
%$$

The reached set of a search tree $\mathcal{T} = (V, E)$, denoted $X_{\mathcal{T}}$, is defined as
\begin{equation}
\label{equation:reachedset}
X_{\mathcal{T}} := \bigcup_{v\in V} \{\overline{x}(v)\}
\end{equation}
which includes all states associated with the vertices in search tree $\mathcal{T}$. An example showing the constructed search graph for solving the sample motion planning problem for the bouncing ball system is given as follows.
\ifbool{conf}{}{
	\begin{example}
		(Bouncing ball system in Example \ref{example:bouncingball}, revisited) Denote the hybrid model of bouncing ball system as $\mathcal{H}$. Figure \ref{figure:propagationsearchgraph} shows the constructed search graph of $\mathcal{H}$ and the corresponding propagation result. The search graph in Figure \ref{figure:searchgraphgraph} is $\mathcal{G} = (V, E)$ where $V =  \{v_{0}, v_{1},..., v_{8}\}$ and $E = \{e_{0}, e_{1},..., e_{7}\}$ such that 
		\begin{equation}
		\begin{aligned}
		e_{0} &= (v_{0}, v_{1})\quad
		e_{1} &= (v_{1}, v_{2})\quad
		e_{2} &= (v_{2}, v_{3})\quad
		e_{3} &= (v_{2}, v_{4})\\
		e_{4} &= (v_{2}, v_{5})\quad
		e_{5} &= (v_{3}, v_{6})\quad
		e_{6} &= (v_{4}, v_{7})\quad
		e_{7} &= (v_{5}, v_{8}).\\
		\end{aligned}
		\end{equation}
		The representation relationships between vertices in Figure \ref{figure:searchgraphgraph} and states in Figure \ref{figure:searchgraphpropagation} are as follows:
		\begin{equation}
		\begin{aligned}
		\overline{x}(v_{0}) &= x_{0}\quad 
		\overline{x}(v_{1}) &= x_{1}\quad 
		\overline{x}(v_{2}) &= x_{2}\quad 
		\overline{x}(v_{3}) &= x_{3}\\
		\overline{x}(v_{4}) &= x_{4}\quad 
		\overline{x}(v_{5}) &= x_{5}\quad 
		\overline{x}(v_{6}) &= x_{6}\quad 
		\overline{x}(v_{7}) &= x_{7}\\
		\overline{x}(v_{8}) &= x_{8}.
		\end{aligned}
		\end{equation}
		The representation relationship between edges in Figure \ref{figure:searchgraphgraph} and solution pairs in Figure \ref{figure:searchgraphpropagation} are as follows:
		\begin{enumerate}
			\item Edge $e_{0} = (v_{0}, v_{1})$ represents the solution pair between $x_{0}$ and $x_{1}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{1} = (v_{1}, v_{2})$ represents the solution pair  between $x_{1}$ and $x_{2}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{2} = (v_{2}, v_{3})$ represents the solution pair  between $x_{2}$ and $x_{3}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{3} = (v_{2}, v_{4})$ represents the solution pair  between $x_{2}$ and $x_{4}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{4} = (v_{2}, v_{5})$ represents the solution pair  between $x_{2}$ and $x_{5}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{5} = (v_{3}, v_{6})$ represents the solution pair  between $x_{3}$ and $x_{6}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{6} = (v_{4}, v_{7})$ represents the solution pair  between $x_{4}$ and $x_{7}$ in \ref{figure:searchgraphpropagation};
			\item Edge $e_{7} = (v_{5}, v_{8})$ represents the solution pair  between $x_{5}$ and $x_{8}$ in \ref{figure:searchgraphpropagation}.
		\end{enumerate}
		The path $p = (v_{0}, v_{1}, v_{2}, v_{3}, v_{6})$ in $\mathcal{G}$ represents the concatenation of $\overline{\psi}(e_{0})$, $\overline{\psi}(e_{1})$, $\overline{\psi}(e_{2})$ and $\overline{\psi}(e_{5})$, namely,
		$$
		\tilde{\psi}(p) = \overline{\psi}(e_{0})|\overline{\psi}(e_{1})|\overline{\psi}(e_{2})|\overline{\psi}(e_{5}).
		$$
		\begin{figure}[htbp]
			\centering
			\subfigure[The search graph of $\mathcal{H}$]{\incfig[0.4]{searchgraphgraph}\label{figure:searchgraphgraph}}
			\subfigure[The corresponding propagation result]{\incfig[0.5]{samplesearchgraphbb}\label{figure:searchgraphpropagation}}
			\caption{The sample search graph}
			\label{figure:propagationsearchgraph}
		\end{figure}
		The reached set $X_{\mathcal{G}} = \{x_{0}, x_{1}, x_{2}, x_{3},x_{4}, x_{5}, x_{6}, x_{7}, x_{8}\}$.
	\end{example}
}



==> section_computation_framework.tex <==
\subsubsection{A computational framework to approximate the simulator of continuous dynamics}
An overall computational approach to approximate the output of simulator of continuous dynamics is introduced in this part. Notations used in the approach are provided as follows.
\begin{enumerate}
	\item The inputs to the simulator of continuous dynamics are the flow set $C$, flow map $f$ and jump set $D$ of the hybrid system $\mathcal{H}$, a priority option flag $rule\in \{flow, jump\}$, $x_{0}\in \overline{C'}$ and $\tilde{u}\in \mathcal{U}_{C}$ such that $(x_{0}, \tilde{u}(0))\in \overline{C}$.
	\item The integration scheme $F_{s}$ (modeled in (\ref{equation:numericalintegrationimplicit})) with its step size $s$ and the zero-crossing detection algorithm $t_{zcd}$ (modeled in (\ref{equation:zerocrossing})) with zero-crossing functions $h_{f}$ and $h_{g}$ are given. Zero-crossing functions $h_{f}$ and $h_{g}$ are constructed given the flow set $C$ and jump set $D$ in the inputs.
	\item The approximation of $\phi$ at $k$th step is denoted as $\phi_{s}(k, 0)$, where $s$ denotes the step size. The value of $u$ at $k$th step is denoted as $u_{s}(k, 0)$, where $s$ denotes the step size.
\end{enumerate} 
Then the computational approach to approximate the output of simulator of continuous dynamics is given in Algorithm \ref{algo:flowsystemsimulator}.
\begin{algorithm}[H]
	\caption{A computational approach to approximate the module $continuous\_simulator$}
	\begin{algorithmic}[1]
		\Function{$continuous\_simulator\_approximate$}{$C, f, D, rule,  x_{0}, \tilde{u}$}
		\State Set $t = 0$, $k = 0$; Set $\phi_{s}(0, 0) = x_{0}$, $u_{s}(0, 0) = \tilde{u}(0)$. 
		\While{$t\leq\overline{t}(\tilde{u})$}
			\State Compute $\phi_{s}(k + 1, 0)$ by solving $F_{s}(\phi_{s}(k, 0), \phi_{s}(k + 1, 0), \tilde{u}, f, t) = 0$.
			\State Set $u_{s}(k + 1, 0) = \tilde{u}(t + s)$.
			\State Set $\hat{t} = t_{zcd} (\phi_{s}(k, 0), \phi_{s}(k + 1, 0), \tilde{u}, t, rule, C, D)$.
			\If{$\hat{t}\neq-1$}
				\State Compute $\phi_{s}(k + 1, 0)$ by solving $F_{\hat{t} - t}(\phi_{s}(k, 0), \phi_{s}(k + 1, 0), \tilde{u}, f, t) = 0$.
				\State Set $u_{s}(k + 1, 0) = \tilde{u}(\hat{t}, 0)$.
				\State $t = \hat{t}$; $k = k + 1$.
				\State break.
			\EndIf
			\State $t = t + s$; $k = k + 1$.
		\EndWhile
		\State \Return $\phi_{s}$, $u_{s}$, $t$, $k$.
		\EndFunction
	\end{algorithmic}
\label{algo:flowsystemsimulator}
\end{algorithm}
The return $(\phi_{s}, u_{s}, t, k)$ of $continuous\_simulator\_approximate(C, f, D, rule,  x_{0}, \tilde{u})$ is a pointwise approximation of the output $(\phi, u)$ of $continuous\_simulator(C, f, D, rule,  x_{0}, \tilde{u})$. For $i = 0, 1, ... k - 1$, $\phi(i\times s, 0) \approx \phi_{s}(i, 0)$ and $u(i\times s, 0) = u_{s}(i, 0)$. For $i = k$, $\phi(t, 0) \approx \phi_{s}(i, 0)$ and $u(t, 0) = u_{s}(i, 0)$.

==> section_numerical_integration.tex <==
\subsubsection{Numerical integration scheme model}
For most systems, the closed-form expression of the integration in (\ref{equation:flowequationintegration}) is not available and the integration has to be computed numerically.

The numerical integration scheme can be modeled as
\begin{equation}
\label{equation:numericalintegrationimplicit}
	F_{s}(x, x^{+}, \tilde{u}, f, t) = 0
\end{equation} where $s$ denotes the step size,  $x$ denotes the state at current step, $x^{+}$ denotes the approximation of state at next step, $\tilde{u}$ denotes the applied input signal, $f$ denotes the flow map, and $t$ denotes the time at current step. $x^{+}$ can be obtained by solving the equation in (\ref{equation:numericalintegrationimplicit}), given $x$, $\tilde{u}$, $f$ and $t$. Two examples on how (\ref{equation:numericalintegrationimplicit}) models explicit and implicit numerical integration scheme are given as follows.
\input{example_fweuler}
\input{example_bweuler}



==> section_zero_crossing_detection.tex <==
\subsubsection{Zero-crossing detection model to approximate $\hat{t}$}
The challenge in implementing Step 2 is to determine $\hat{t}$ in (\ref{equation:integrationduration}) during the integration. When $rule$ equals $flow$, $\hat{t}$ is the first time when $(\hat{\phi}, \tilde{u})$ steps outside set $C$. When $rule$ equals $jump$, $\hat{t}$ is the first time when $(\hat{\phi}, \tilde{u})$ steps outside set $C\backslash D$.

When $rule = flow$, if there exists a zero-crossing function $h_{f}: \mathbb{R}^{n}\times \mathbb{R}^{m}\to \mathbb{R}$ for the given flow set $C$ such that 
	\begin{enumerate}
		\item $h_{f}(x, u) > 0$ for all $(x, u)\in \interior C$,
		\item $h_{f}(x, u)< 0$ for all $(x, u)\in \interior (\mathbb{R}^{n}\times \mathbb{R}^{m}\backslash C)$,
		\item $h_{f}(x, u) = 0$ for all $(x, u)\in \partial  C$,
		\item $h_{f}$ is continuous over $\mathbb{R}^{n}\times \mathbb{R}^{m}$,
\end{enumerate}
then $\hat{t}$ is the first time when $h_{f}(\hat{\phi}, \tilde{u})$ crosses zeroes and can be approximated by zero-crossing detection algorithm. 

When $rule = jump$, if there exists a zero-crossing function $h_{g}: \mathbb{R}^{n}\times \mathbb{R}^{m}\to \mathbb{R}$ for the given flow set $C$ and jump set $D$ such that 
	\begin{enumerate}
			\item $h_{g}(x, u) > 0$ for all $(x, u)\in \interior (C\backslash D)$,
		\item $h_{g}(x, u)< 0$ for all $(x, u)\in \interior (\mathbb{R}^{n}\times \mathbb{R}^{m}\backslash (C\backslash D))$,
		\item $h_{g}(x, u) = 0$ for all $(x, u)\in \partial  (C\backslash D)$,
		\item $h_{g}$ is continuous over $\mathbb{R}^{n}\times \mathbb{R}^{m}$,
	\end{enumerate}
	then $\hat{t}$ is the first time when $h_{g}(\hat{\phi}, \tilde{u})$ crosses zeroes and can be approximated by zero-crossing detection algorithm.
\begin{example}
	(Bouncing ball system in Example \ref{example:bouncingball}, revisited) In the bouncing ball system, the flow set is $C = \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1}\geq 0\}$ and jump set is $D = \{(x, u) \in \mathbb{R}^{2}\times \mathbb{R}: x_{1} = 0, x_{2} \leq 0, u\geq 0\}$. Then $h_{f}$ can be designed as:
	\begin{equation}
		h_{f}(x, u): = x_{1}\quad (x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}.
	\end{equation} 
	Note that $D\subset \partial C$. Therefore, $\interior (C\backslash D) = \interior C$ and $\interior (\mathbb{R}^{n}\times \mathbb{R}^{m}\backslash (C\backslash D)) = \interior (\mathbb{R}^{n}\times \mathbb{R}^{m}\backslash C)$. Therefore, $h_{g}$ can be designed in the same way as $h_{f}$:
	\begin{equation}
		h_{g}(x, u): = x_{1}\quad (x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}.
	\end{equation}
\end{example}

The zero-crossing detection algorithm that approximates $\hat{t}$ can be modeled as 
\begin{equation}
	\label{equation:zerocrossing}
	\hat{t} = t_{zcd} (x, x^{+}, \tilde{u}, t, rule, C, D)
\end{equation}
where $x$ and $x^{+}$ denote states at consecutive steps obtained by numerical integration, $\tilde{u}$ denotes the applied input signal, $t$ denotes the time at current step, $rule$ denotes the priority option and $C$ and $D$ denotes the flow set and jump set of the given hybrid system. The zero-crossing functions $h_{f}$ and $h_{g}$ are constructed based on $C$ and $D$. $\hat{t}$ is set to $-1$ when no zero-crossing is detected.



==> sections/section3/main.tex <==
\input{chapters/chapter6/preliminariessampling}
	\input{chapters/chapter6/searchbasedinputlibrary}
	\input{chapters/chapter6/searchbasedcontinuoussimulator}
	\input{chapters/chapter6/searchbaseddiscretesimulator}
	\input{chapters/chapter6/searchgraph}
	\input{chapters/chapter6/samplingbasedalgorithm}
%\section{Time complexity analysis}
%\input{chapters/chapter6/computationcomplexity.tex}
%\section{Examples}
%\input{chapters/chapter6/examples.tex}
\section{\textbf{Task 5}: Closeness between the results of the theoretical algorithms and their numerical implementation}
\input{chapters/chapter6/task1.tex}
\section{Research progress of the work in this thrust}
We have completed the tasks 1 - 4 for implementing Algorithm \ref{algo:theoreticalalgo} proposed in Thrust 1. Note that the algorithms to be proposed in Thrusts 2 and 3 are also graph-based, therefore, most of the results in tasks 1 - 4 above will be reused in implementing those algorithms with slight changes. We plan to justify Assumption \ref{assumption:closeness} for the implementation of Algorithm \ref{algo:theoreticalalgo} and the algorithms to be proposed in Thrusts 2 and 3. 


==> simulators.tex <==
\input{continuoussimulator}
\input{discretesimulator}
